Bottom Up Top Down Detection Transformers for Language Grounding in Images and Point Clouds

Most models tasked to ground referential utterances in 2D and 3D scenes learn to select the referred object from a pool of object proposals provided by a pre-trained detector. This is limiting because an utterance may refer to visual entities at various levels of granularity, such as the chair, the leg of the chair, or the tip of the front leg of the chair, which may be missed by the detector. We propose a language grounding model that attends on the referential utterance and on the object proposal pool computed from a pre-trained detector to decode referenced objects with a detection head, without selecting them from the pool. In this way, it is helped by powerful pre-trained object detectors without being restricted by their misses. We call our model Bottom Up Top Down DEtection TRansformers (BUTD-DETR) because it uses both language guidance (top down) and objectness guidance (bottom-up) to ground referential utterances in images and point clouds. Moreover, BUTD-DETR casts object detection as referential grounding and uses object labels as language prompts to be grounded in the visual scene, augmenting supervision for the referential grounding task in this way. The proposed model sets a new state-of-the-art across popular 3D language grounding benchmarks with significant performance gains over previous 3D approaches (12.6% on SR3D, 11.6% on NR3D and 6.3% on ScanRefer). When applied in 2D images, it performs on par with the previous state of the art. We ablate the design choices of our model and quantify their contribution to performance. Our code and checkpoints can be found at the project website https://butd-detr.github.io.

==> 0_abstract_old.tex <==
\begin{abstract}

%Language grounding models are tasked to localize the entities in the input scene that the  language   utterance refers to. 
Most language grounding models learn to select the referred object from a pool of object proposals provided by a pre-trained detector. 
This object proposal bottleneck is limiting because an utterance may refer to visual entities at various levels of granularity, such as the chair, the leg of a chair, or the tip of the front leg of a chair, which may be missed by the  detector. 
%Object detectors are typically trained on a fixed vocabulary of objects and attributes that is often too restrictive for open-domain language grounding.  
 Recently,  MDETR \cite{Kamath2021MDETRM} introduced a language grounding model for 2D images that does not have such a box proposal bottleneck; instead of selecting objects from a proposal pool, it instead decodes the referenced object boxes directly from image and language features, and achieves big leaps in performance.   %  a DETR object detection head \cite{Carion2020EndtoEndOD}. % using image and referential utterance as input.  % through  cross-attention between vision and language features and box-span alignment losses.
 We propose a language  grounding model for 3D scenes  built on MDETR, which we call Bottom Up Top Down DEtection TRansformer (BUTD-DETR). % \underline{B}\underline{U}\underline{T}\underline{erD}-DETR,  from \underline{b}ottom-\underline{u}p and \underline{t}op-\underline{d}own DETR.   %The proposed model also
% We call our model \underline{B}EA\underline{U}\underline{T}Y-\underline{D}ETR,  as it uses both box  proposals, obtained by a general purpose detector  ``\underline{bo}ttom-\underline{u}p", and ``\underline{t}op-\underline{d}own" guidance from the  language utterance, to decode the referenced objects in the scene. 
 \model{} attends on an additional object proposal pool computed bottom-up from a pre-trained detector. Yet it  decodes referenced objects  without  selecting them from the pool. In this way it  uses powerful object detectors to help ground language without being restricted by their misses.   
 Second, \model{}  augments  supervision  from language grounding annotations by configuring object detection annotations as language prompts to be grounded in images. %The two innovations, inclusion of a bottom-up stream and supervision from detection prompts, alongside other architectural innovations,  
 %is co-trained for grounding 
 %It learns to infer 3D object boxes for the referred entities 
 %modulates 3D object detectors through attention to the input referential language utterance 
 %and has the following innovations over its 2D counterpart: 
 %It outperforms 
 %i) It uses an additional object proposal stream  to attend to without being restricted to select its answer from. ii) It is co-trained from object detection annotations  by supplying a list of category labels as the referential utterance to be grounded. 
 %iii) It has improved and more computational viable attention operations across vision, language and box streams. \todo{new loss is more important}
 The proposed model sets a new state-of-the-art across  %benefits from already available strong detectors and deetction supervision
%shows significant performance gains  over previous approaches on 
popular 3D language grounding benchmarks with significant performance gains over previous 3D approaches (12.6\% on SR3D, 11.6\% on NR3D and 6.3\% on ScanRefer). It outperforms a straightforward 3D MDETR implementation  by 6.7\% on SR3D, 11.8\% on NR3D and 5\% on ScanRefer benchmarks. 
When applied on language grounding in 2D images, it performs  on par with MDETR.
%and converges  in  half of the GPU time thanks to architectural and loss optimizations. 
We ablate each of the design choices  of the model and  quantify their contribution to performance.

%The project website at \url{https://butd-detr.github.io} includes code and checkpoints for our model. 

%Project website, also including code and checkpoints, at \url{https://butd-detr.github.io}.
\end{abstract}


==> OLD2_related.tex <==
\section{Related work}



\subsubsection{Object detection with transformers}
%Object detection is a classic computer vision task 
%where a closed set of object category labels is considered and 
%instances of those labels are localized with bounding boxes and segmentations in the image. Then, a
Object detectors are trained  
%the detection model is tasked 
to localize all instances of a closed set of object category labels in images and 3D point-clouds. While earlier architectures  pool features within proposed boxes to decode objects and classify them into categories %  and classification heads over convolutional variants of image encoders
\cite{DBLP:journals/corr/HeGDG17,DBLP:journals/corr/LiuAESR15,Redmon2016YouOL},  recent methods pioneered by DETR \cite{Carion2020EndtoEndOD} use transformer architectures where a set of object query vectors attend to the scene and among themselves to decode object boxes and their labels. DETR suffers from quadratic cost of within  image features  self attention.  D(eformable)-DETR \cite{Zhu2021DeformableDD} proposes  deformable attention, a locally adaptive kernel that is predicted directly in each pixel location without attention to other pixel locations, thus saving the quadratic cost of pixel-to-pixel attention, by noting that content-based attention does not contribute significantly in performance \cite{Zhu2019AnES}. Our model builds upon deformable attention  for feature extraction from RGB images. %\todo{$<-$ this does not fit here}    %and unsupervised pretraining \cite{Dai2020UPDETRUP}
%of such transformer-based object detector by proposing deformable attention, a locally adaptive kernel that is predicted directly in each pixel location, without cross-attention to other locations, 
The works of \cite{Liu2021GroupFree3O} and \cite{Misra2021AnET} extend transformer encoders and detector heads to 3D point cloud input. 


\subsubsection{2D referential language grounding}
Referential language grounding \cite{Kazemzadeh2014ReferItGameRT} is the task  of  localizing the object(s) referenced in a language  utterance. %,  was introduced to handle the limitation of  generic object detectors to reference visual entities relevant for a task yet absent from a general vocabulary.  
%In close inspection, object annotations of a particular object category can be treated as annotations for the grounding task where the referential utterance is a single word, namely, the category label itself;  this is precisely exploited by BEAUTY-DETR in co-training with detection prompts. \todo{this paragraph does not sound as related work to me}
%The ability to  localize objects mentioned in an utterance  is central for an intelligent agent to communicate, learn and be instructed by humans. There is a lot of research on models for language grounding that fuse information across image and language streams. 
%For ease of exposition, we group existing models into three broad categories based on whether they pursue or not a generic, task-independent, visual tokenization of the scene: 
%i) 
Most 2D language grounding models  obtain  sets of object proposals using  pre-trained  object detectors and  the original image is discarded upon extraction of the object proposals %, i.e., the visual tokens  %before fusing visual and language modalities 
\cite{fang2015captions,densecap,karpathy2015deep2,Fukui2016MultimodalCB,modularreferential}. Many  approaches use multiple layers of attention  %, already tremendously successful in natural language processing \cite{Devlin2019BERTPO},
to fuse information across both the extracted boxes and language utterance \cite{Lu2019ViLBERTPT,Chen2020UNITERUI,Yang2021SAT2S}.  
%to  localize referent objects or answer questions about an image \cite{Lu2019ViLBERTPT,Chen2020UNITERUI,Yang2021SAT2S}.  
%Instead of transformer layers, neural-symbolic approaches  use 
Neural symbolic methods infer programs of neural modules that are applied on the extracted box proposals and their color and shape descriptors  \cite{Yi2018NeuralSymbolicVD,Mao2019NeuroSymbolic}. 
%by mapping the utterance to a computational graph over  modules and applying it to  the disentangled visual representation.
These latter models have been mainly applied in  domains where the computational graph to answer a question or find an object is well-defined such as CLEVR \cite{DBLP:journals/corr/JohnsonHMFZG16} or CLEVRER \cite{DBLP:journals/corr/abs-1910-01442}. %, where the computational graph to answer a question or find an object is well-defined and an accurate  tokenization of the scene can be obtained with existing object detectors. 
%This is clearly not the case for our Figure \ref{fig:overview} where detectors cannot obtain a clean visual decomposition. 
Modular network architectures  \cite{andreas-etal-2016-learning,hu2017learning,DBLP:journals/corr/JohnsonHMHLZG17,chen2021meta} predict a computational graph given the input utterance and process the input image as directed by the inferred computational graph, which may involve applying detectors or masking operations in specific locations. They do not require an extraction of box proposals beforehand to select from. % tokenization of the image into objects. 
%grid-based image patch extraction 
%ii) Models that do not tokenize the visual scene but rather apply operations directly on pixels to extract relevant information, 
%either end-to-end \cite{Lu2016HierarchicalQC,Xu2015ShowAA}  MDETR is one of the latest products of this line of work with state-of-the-art performance across multiple 2D grounding datasets. 
%iii) 

Our work builds upon MDETR of Kamath et al. \cite{Kamath2021MDETRM} that modulates visual processing through attention to the input language utterance and decodes objects from queries similar to DETR, without selecting them from a pool of proposals.  %\todo{depending on results we may want to say we dont want to learn detection from scratch}. % Our work extends language modulated detection to the 3D domain and improves the computational cost of language modulated detectors in the 2D domain.

%Our method attends directly on the visual stream (points/pixels) and thus does not have a detection bottleneck. At the same time, it does not discard the easy-to-detect proposals from an object detector.



   \subsubsection{3D referential language grounding} has only recently gained popularity \cite{Chen2020ScanRefer3O,Achlioptas2020ReferIt3DNL}. To the best of our knowledge, all related approaches are box-bottlenecked: they first extract 3D object proposals and then select one as their answer. Their pipeline can be decomposed into three main steps: i) Representation of object boxes as point features \cite{Yang2021SAT2S}, segmentation masks \cite{Yuan2021InstanceReferCH} or pure spatial/categorical features \cite{Roh2021LanguageReferSM}. ii) Encoding of language utterance using word embeddings \cite{Yang2021SAT2S,Roh2021LanguageReferSM} and/or scene graphs \cite{Feng2021FreeformDG}. iii) Fusion of the two modalities and scoring of each proposal using graph networks \cite{Huang2021TextGuidedGN} or Transformers \cite{Yang2021SAT2S}. Most of these works also employ domain-specific design choices by explicitly encoding pairwise relationships  \cite{Huang2021TextGuidedGN,he2021TransRefer3DEA,Yuan2021InstanceReferCH} or by relying on heuristics, such as restricting attention to be local \cite{Zhao_2021_ICCV,Yuan2021InstanceReferCH} and ignoring input modalities \cite{Roh2021LanguageReferSM}. Such design choices prevent those architectures from being applicable to both the 3D and 2D domains simultaneously.
    
    Due to the inferior performance of 3D object detectors in comparison to their 2D counterparts, popular benchmarks for 3D language grounding, such as Referit3D \cite{Achlioptas2020ReferIt3DNL} provide access to ground-truth object boxes at test time. The proposed $\model$ is the first 3D language grounding model that is evaluated on this benchmark without access to  oracle 3D object boxes. %Furthermore, our model also outperforms previous state-of-the-art models with huge margin even in the original benchmark setting of ground truth detection. \todo{that's great but this is a claim/contribution}   % Co-training of our model under both object detection and referential grounding objectives gives a significant boost over training for grounding alone. In addition, our design is not domain-specific and our model can work for both 3D and 2D scenes. Lastly, while previous 3D approaches score a set of proposals to return only one answer matching the ``root'' noun phrase, our model predicts boxes and corresponding spans and can thus output all mentioned objects.
 

==> notes.tex <==

\begin{comment}



To investigate performance of $\model$ in the presence and absence of good box proposals in the box proposal stream, we report performance of i) the full model, ii) a corresponding box-bottlenecked model that does not attend on point features, iii) does not decode boxes but rather selects the box from the box proposal pool, which is similar to LanguageRefer \cite{Roh2021LanguageReferSM}, and iv) a top-down $\model$ that does not attend on a box stream in Table~\ref{table:accuracy_}. 
%To further investigate the contribution of each attention stream, in Table~\ref{table:accuracy_}
We measure the recall of each model, as the percentage of times any predicted box is successful, and we report results for both the cases when the detector is successful as well as when it is not. We draw the following conclusions:
\begin{itemize}
    \item When the pre-train detector misses the referred object,  $\model$ is successful in recovering the object 16.1\% of the cases,  a box-bottlenecked  model can never recover and the top-down model is successful in recovering the object 22.4\% of the cases. 
    \item When the pre-train detector detects the referred object,  $\model$ still outperforms the box-bottlenecks model, potentially from its ability to refine the box, and also outperforms the top-down model.
    \item In aggregate, $\model$ outperforms its top down counterpart by 2\% and converges in less than half the number of epochs. % its box-bottneklec counterpart 
    %is successful in recovering the object 16.1\% of the cases, while a box-bottlenecked  model can never recover. 
\end{itemize}

\end{comment}





\begin{comment}


% \vspace{-2em}

\subsection{Implementation Details}
In 3D, the input point cloud is encoded with PointNet++ \cite{Qi2017PointNetDH} using the same hyperparameters as in \cite{Liu2021GroupFree3O}, pre-trained on ScanNet \cite{Dai2017ScanNetR3}. We use the last layer's features, resulting in 1024 visual tokens. 
In the decoder, the object queries are formed from the 256 most confident visual tokens. We set $N_E=3$ with no self-attention layers, $N_D=6$. All attention layers are implemented using standard self-/cross-attention.
In 2D, we encode the image using a pre-trained ResNet-101. We set $N_E=6$ and $N_D=6$. All attention layers to the visual stream are implemented with deformable attention \cite{Zhu2021DeformableDD}, attention to other the language stream or detected boxes is the standard attention of \cite{Vaswani2017AttentionIA,Lu2019ViLBERTPT}. For more implementation details please see the supplementary file.
\end{comment}
